Domain Knowledge Graph Construction Via A Simple Checker

With the availability of large language models, there is a growing interest for semiconductor chip design companies to leverage the technologies. For those companies, deployment of a new methodology must include two important considerations: confidentiality and scalability. In this context, this work tackles the problem of knowledge graph construction from hardware-design domain texts. We propose an oracle-checker scheme to leverage the power of GPT3.5 and demonstrate that the essence of the problem is in distillation of domain expert's background knowledge. Using RISC-V unprivileged ISA specification as an example, we explain key ideas and discuss practicality of our proposed oracle-checker approach.

==> mainApp7andApp8.tex <==
\subsection{Cross-Paragraph Connections}
\label{App.07}


\begin{figure*}[htb]
	%#P18
	\centering
	%\includegraphics[width=2.2in]{Figures/fig08.pdf}
	\includesvg[inkscapelatex=false, width=6.5in]{Figures/figApp01.svg}
	\includesvg[inkscapelatex=false, width=6.5in]{Figures/figApp02.svg}
	\vspace{-0.5cm}
	\caption{\small \textbf{Top} (BF$\phi$): 67 concepts shared by at least the RDFs of two paragraphs with 
	the total number of 320 connections shown in the bipartite graph; Note that this result includes
	all RDFs even though they fail the entailment check; \textbf{{Bottom} (BF$A$): 75 concepts shared by at least two paragraph and the total number of connections increases to 454; In the bipartite graphs, the
    bottom dots each represents a paragraph from chapter 1 and the upper squares each represents a subject entity}
	\label{figApp01} 
	\vspace{-0.2cm}
\end{figure*}

\begin{figure*}[htb]
	%#P18
	\centering
	%\includegraphics[width=2.2in]{Figures/fig08.pdf}
	\includesvg[inkscapelatex=false, width=6.5in]{Figures/figApp03.svg}
	\includesvg[inkscapelatex=false, width=6.5in]{Figures/figApp04.svg}
	\vspace{-0.5cm}
	\caption{\small \textbf{Top} (BF$\phi$): 72 concepts shared by at least the RDFs of two paragraphs with 
		the total number of 307 connections shown in the bipartite graph; Note that this result includes
		all RDFs even though they fail the entailment check; \textbf{Top} (BF$A$): 82 concepts shared by at least two paragraph and the total number of connections increases to 388; In the bipartite graphs, the
		bottom dots each represents a paragraph from chapter 2 and the upper squares each represents a subject entity}
	\label{figApp03} 
	\vspace{-0.2cm}
\end{figure*}

A total of 433 and 591 subject entities are extracted for chapter 1 
from BF$\phi$ and BF$A$, respectively. 
A total of 452 and 577 subject entities are extracted for chapter 2 
from BF$\phi$ and BF$A$, respectively.

We use a simple method to group the subject entities 
into high-level subject concepts.
We observed that the suffix word of a subject entity phrase usually 
captures the high-level meaning of the phrase. For example, 
``CSRInstruction" and ``StoreInstruction" both belong to the concpet of 
``Instruction". 
Suffix can be easily split from the entity phrase since RDF
already formats the phrases into Camel or Snake case. 
We further use a stemming tool \cite{nltk-stemmer} to remove morphological affixes from the suffix words
so that words with the same stem will be grouped together. For example, 
``encodings" and ``encodes" belong to the same group. 

The subject concepts serve two purposes: (1) to create an ontology 
vocabulary that can be used to group concepts. For
example, ``Instruction" is an ontology term that groups
``CSRInstruction" and ``StoreInstruction". (2)
to reduce the number of different concepts and 
facilitate the display of results shown in Figure \ref{figApp01} and
Figure \ref{figApp03}

For chapter 1, we collected a total of 168 and 178 subject concepts 
from BF$\phi$ and BF$A$, respectively. These subject concepts show 
421 and 557 occurrences in paragraphs for BF$\phi$ and BF$A$, respectively. 
Figure \ref{figApp01} shows bipartite graphs of 
the subject concepts that appear in at least two paragraphs
for chapter 1. 
For chapter 2, we collected a total of 211 and 191 subject concepts 
from BF$\phi$ and BF$A$, respectively. These subject concepts show 
446 and 497 occurrences in paragraphs for BF$\phi$ and BF$A$, respectively. 
Figure \ref{figApp03} shows bipartite graphs of 
the subject concepts that appear in at least two paragraphs
for chapter 2.

Table \ref{tableApp01} shows the top five subject concepts 
that have the highest
connectivity (the highest number of occurrences) 
in Figure \ref{figApp01} (top). 
The subject entities that are grouped
under the concept are also listed. 
Table \ref{tableApp02} shows the concpets and the corresponding entities
for Figure \ref{figApp01} (bottom).
Table \ref{tableApp03} shows the concpets and the corresponding entities
for Figure \ref{figApp03} (top).
Table \ref{tableApp04} shows the concpets and the corresponding entities
for Figure \ref{figApp03} (bottom).

\begin{table*}[htb]
    \centering
    \begin{tabular}{c|l}
        \textbf{Subject Concept} & \textbf{BF$\phi$ Subject Entities}    \\ \hline
        Instruction (23)  &  New\_Instructions, cacheControlInstruction, \\
                          & fenceInstruction, StoreInstruction, IllegalInstructions\\
                          & specificInstructions, Variable\_Length\_Instructions, \\
                          &  32\_bit\_instruction, Optional\_Longer\_Instructions,  \\
                          &  LittleEndianInstruction, ErrorfulInstruction, \\
                          & unprivilegedInstructions, Instruction, MachineInstruction,\\
                          & optional\_compressed\_instruction, LoadInstruction \\ \hline
        Trap (19) & Opcode\_Traps, Trap, InvisibleTrap, RequestedTrap, \\
                  & FatalTrap, ContainedTrap \\ \hline
        ISA (19) & RISC-V\_ISA, Base\_Integer\_ISA, Base\_ISA, singleISA, ISA, \\
                 & whyNotSingleISA, Unprivileged\_ISA \\ \hline 
        Extension (16) & Additional\_Instruction\_Set\_Extension, \\
                       & Specialized\_Instruction\_Set\_Extension, \\
                       & Optional\_Extension, nonConformingExtension, \\
                       & InstructionSetExtensions, Subsequent\_Extensions, \\
                       & GC\_Extensions, Standard\_Compressed\_ISA\_Extension, \\
                       & StandardExtensions, StandardInstructionSetExtension, \\
                       & compressed\_instruction\_set\_extensions, \\
                       & OtherExtensions, nonStandardExtension, Extensions\\ \hline
        Execution Environment (15) & Software\_Execution\_Environment, \\
                                   & Hardware\_Execution\_Environment, \\
                                   & RISC-V\_Execution\_Environment, \\
                                   & Hardware\_and\_Software\_Execution\_Environment, \\
                                   & BareMetalEnvironment, Execution\_Environment\\
                                   & OperatingSystemEnvironment \\ \hline



    \end{tabular}
    \caption{\small BF$\phi$ Entities from Chapter 1 with top occurrences. 
    The first column shows the domain suffix term that is shared by the entities.   
    The number in parenthesis indicates the number of paragraphs where the phrase occurs.}
    \label{tableApp01}
\end{table*}

\begin{table*}[htb]
    \centering
    \begin{tabular}{c|l}
        \textbf{Subject Concept} & \textbf{BF$\phi$ Subject Entities}    \\ \hline
        Extension (38) & Instruction\_Set\_Extension, Extension, nonStandardExtension,\\
                       & vendorSpecificNonStandardExtension, compressed\_extension, \\
                       & standard\_GC\_extensions, Compressed\_ISA\_Extension, \\
                       & customExtension, StandardCompressedInstructionExtension,\\ 
                       & StandardLargerThan32BitInstructionSetExtension, \\
                       & NonConformingExtension, StandardFloatingPointExtension, \\
                       & openToExtensions, ISA\_Extension, \\
                       & OtherExtensions, has\_extension \\ \hline
        ISA (33) & ISA, RISC-V\_ISA, has\_base\_ISA, Base\_Integer\_ISA, unifiedISA, \\ 
                 & not\_treating\_design\_as\_single\_ISA, Unprivileged\_ISA, \\
                 & standard\_IMAFD\_ISA, singleISA, notSingleISA \\ \hline
        Trap (33) & Trap, differences\_in\_addressing\_and\_illegal\_instruction\_traps, \\
                  & illegal\_instruction\_traps, NoTrap, FatalTrap, ContainedTrap, \\
                  & RequestedTrap, DefinedSolelyToCauseRequestedTraps,  \\
                  & InvisibleTrap, OpcodeTrap \\ \hline
        Instrucion (31) & RISCVBaseInstructions, MultiplicationInstruction, \\
                        & DoublePrecisionInstruction, ControlFlowInstruction, \\
                        & IntegerComputationalInstruction, SinglePrecisionInstruction, \\
                        & DivisionInstruction, AtomicInstruction, CompressedInstruction, \\
                        & LoadInstruction, Instruction, MachineInstruction\\
                        & Compressed\_16\_Bit\_Instruction, 32\_Bit\_Instruction, \\
                        & illegal\_30\_bit\_instructions, illegalInstruction, 16BitInstruction, \\
                        & AllZeroBitsInstruction, Variable-Length\_Instruction, \\
                        & AllOnesInstruction, KnownErrorfulInstructions, StoreInstruction, \\
                        & MissingInstruction, UnprivilegedInstructions, CommonInstruction\\ \hline
        Execution Environment (15) & HardwareAndSoftwareExecutionEnvironment, \\
                                   & SoftwareExecutionEnvironment, \\
                                   & SupervisorLevelExecutionEnvironment, \\
                                   & UserLevelExecutionEnvironment, OuterExecutionEnvironment, \\
                                   & BareMetalEnvironment, ExecutionEnvironment \\ \hline 
        Hart (15) & Hart, HostHart, GuestHart, EachHart, AllHarts \\ \hline 
    \end{tabular}
    \caption{\small BF$A$ Entities from Chapter 1 with top occurrences. }
    \label{tableApp02}
\end{table*}

\begin{table*}[htb]
    \centering
    \begin{tabular}{c|l}
        \textbf{Subject Concept} & \textbf{BF$\phi$ Subject Entities}    \\ \hline
        Instruction (23) & CSRInstructions, systemInstructions, CurrentInstruction, 16BitInstructions, \\
                         & Jump\_Instruction, Branch\_Instruction, Conditional\_Branch\_Instruction, \\
                         & Instruction, LoadUpperImmediateInstruction, RegularInstruction, \\
                         & hasInstruction, IntegerComputationalInstructions, \\
                         & SingleAdditionalBranchInstruction, AdditionalInstructions, \\
                         & ControlTransferInstructions, unconditionalJumpInstructions, \\
                         & ConditionalBranchInstruction, 16BitAlignedInstructions, \\
                         & AddressOfBranchInstruction, PredicatedInstructions \\ \hline
        Format (19) & InstructionFormat, 3AddressFormat, 2AddressFormat, S\_Format, R\_Format, \\
                    & U\_Format, I\_Format, B\_InstructionFormat, J\_InstructionFormat, B\_format,\\
                    & Base\_Instruction\_Formats, usesFormat, JTypeFormat, BTypeInstructionFormat \\ \hline
        Register (12) & numberOfRegisters, 32IntegerRegisters, IntegerRegisters, hasDestinationRegister, \\
                      & placesResultInRegister, AlternateLinkRegister, RegularReturnAddressRegister,\\
                      & GeneralPurposeRegister, linkRegister, TwoRegisters \\ \hline
        ISA (9) & baseIntegerISA, integerISA, completeISA, RV32I\_ISA, BaseISA, ISA \\ \hline 
        Extension (9) & OtherISAExtensions, InstructionSetExtension, NonConformingExtension, \\
                      & CompressedInstructionSetExtension, AExtension, Extension \\ \hline 
    \end{tabular}
    \caption{\small BF$\phi$ Entities from Chapter 2 with top occurrences.}
    \label{tableApp03}
\end{table*}

\begin{table*}[htb]
    \centering
    \begin{tabular}{c|l}
        \textbf{Subject Concept} & BF$A$ \textbf{Subject Entities}    \\ \hline
        Instruction (23) & CSRInstructions, ConditionalBranchInstruction, BranchInstruction, \\
                         & reservedInstruction, regular\_instruction, load\_upper\_immediate\_instruction, \\
                         & IntegerComputationalInstruction, JumpInstruction, AdditionalInstructions, \\
                         & LoadStoreInstructions, ControlTransferInstructions, \\
                         & unconditionalJumpInstructions, PredicatedInstructions, \\ \hline
        Immediate (17) & 5-bit\_Immediate, Immediate, J\_immediate, J\_shifted\_immediate, \\ 
                       & 20\_bit\_immediate, U\_immediate, U\_shifted\_immediate \\ \hline 
        ISA (16) & SubsetOfBaseIntegerISA, ISA, BaseIntegerISA, RISC-V\_ISA, \\
                 & Unprivileged\_State\_for\_Base\_Integer\_ISA, Complete\_Set\_of\_Base\_Integer\_ISA, \\ 
                 & integer\_ISA, baseISA \\ \hline 
        Register (15) & CSRRegisters, hasNoStackPointerOrSubroutineReturnAddressLinkRegister, \\
                      & usesRegisterX5AsAlternateLinkRegister, 16\_registers, number\_of\_registers, \\
                      & larger\_number\_of\_integer\_registers, integer\_register, \\
                      & frequently\_accessed\_registers, returnAddressRegister \\ \hline 
        Format (12) & InstructionFormat, 2-address\_format, OptionalCompressed16BiatInstructionFormat, \\ 
                    & CoreInstructionFormat, B\_format, S\_format, U\_format, J\_format, \\
                    & BaseInstructionFormats, BTypeInstructionFormat, alternateLinkRegister, \\
                    & ReturnAddressRegister \\ \hline 
    \end{tabular}
    \caption{\small BF$A$ Entities from Chapter 2 with top occurrences.}
    \label{tableApp04}
\end{table*}

\subsection{Background Facts}
\label{App.08}

The 204 manually created background facts are listed in Figure \ref{figApp05}, \ref{figApp06}, and \ref{figApp07}.

\begin{figure*}[htb]
	\centering
	%\includegraphics[width=2.2in]{Figures/fig08.pdf}
	\includesvg[inkscapelatex=false, width=6.5in]{Figures/figApp05.svg}
	\vspace{-0.2cm}
	\caption{\small Background facts}
	\label{figApp05} 
	\vspace{-0.2cm}
\end{figure*}

\begin{figure*}[htb]
	\centering
	%\includegraphics[width=2.2in]{Figures/fig08.pdf}
	\includesvg[inkscapelatex=false, width=6.5in]{Figures/figApp06.svg}
	\vspace{-0.2cm}
	\caption{\small Background facts Cont'd}
	\label{figApp06} 
	\vspace{-0.2cm}
\end{figure*}

\begin{figure*}[htb]
	\centering
	%\includegraphics[width=2.2in]{Figures/fig08.pdf}
	\includesvg[inkscapelatex=false, width=6.5in]{Figures/figApp07.svg}
	\vspace{-0.2cm}
	\caption{\small Background facts Cont'd}
	\label{figApp07} 
	\vspace{-0.2cm}
\end{figure*}



